Spacetime aspects of non-supersymmetric strings

The consistency of string theory as a theory of gravity does not rely on the presence of spacetime supersymmetry; however, its absence leads to the emergence of tadpole diagrams in the on-shell worldsheet formulation, thus undermining our control over the physics. Two-dimensional conformal invariance, a pillar of string theory, requires tadpole subtraction through the Fischler-Susskind mechanism, whose spacetime consequence is the emergence of scalar tadpole potentials. In this thesis, I explore several implications of the absence of supersymmetry in string-derived scenarios. I focus on the three ten-dimensional tachyon-free string theories in which spacetime supersymmetry is absent or broken, studying the gravitational consequences of tadpole potentials. First, I address vacuum solutions in terms of singular codimension-one vacua, explore their generalizations, and discuss the properties of their singular boundaries. I present an alternative perspective on these vacua based on the formalism of fake supersymmetry, in which the second-order equations of motion are replaced by supersymmetry-like first-order equations. I then turn to the topic of engineering vacua in the non-supersymmetric string models by constructing solutions that are supported by electric and magnetic fluxes and by providing evidence for their instability. Finally, I investigate brane-like solutions in the presence of tadpole potentials that yield both flux vacua with the isometries of supersymmetric branes and gravitational profiles that capture the backreaction of localized sources.

==> endmatter/colophon.tex <==
%!TEX root = ../dissertation.tex
\newpage

% If you do want an image in the colophon:
% \begin{figure}
%   \vspace{20pt}
%   \centering
%   \hspace*{-32pt}
%   \includegraphics[width=0.42\textwidth]{endmatter/colophon.png}
% \end{figure}

% If you don't want an image in the colophon:
\vspace*{200pt}

\begin{center}
\parbox{400pt}{\lettrine[lines=3,slope=-2pt,nindent=-4pt]{\textcolor{SchoolColor}{T}}{his thesis was typeset} using \LaTeX, originally developed by Leslie Lamport and based on Donald Knuth's \TeX. The body text is set in 11 point Egenolff-Berner Garamond, a revival of Claude Garamont's humanist typeface. A template that can be used to format a PhD dissertation with this look \textit{\&} feel has been released under the permissive \textsc{agpl} license, and can be found online at \href{https://github.com/suchow/Dissertate}{github.com/suchow/Dissertate} or from its lead author, Jordan Suchow, at \href{mailto:suchow@post.harvard.edu}{suchow@post.harvard.edu}.}
\end{center}


==> endmatter/personalize.tex <==
%!TEX root = ../dissertation.tex


==> frontmatter/abstract.tex <==
%!TEX root = ../dissertation.tex
% the abstract

The consistency of string theory as a theory of gravity does not rely on the presence of spacetime supersymmetry; however, its absence leads to the emergence of tadpole diagrams in the on-shell worldsheet formulation, thus undermining our control over the physics.
Two-dimensional conformal invariance, a pillar of string theory, requires tadpole subtraction through the Fischler-Susskind mechanism, whose spacetime consequence is the emergence of scalar \emph{tadpole potentials}.
In this thesis, I explore several implications of the absence of supersymmetry in string-derived scenarios. I focus on the three ten-dimensional tachyon-free string theories in which spacetime supersymmetry is absent or broken, studying the gravitational consequences of tadpole potentials.
First, I address vacuum solutions in terms of singular codimension-one vacua, explore their generalizations, and discuss the properties of their singular boundaries.
I present an alternative perspective on these vacua based on the formalism of \emph{fake supersymmetry}, in which the second-order equations of motion are replaced by supersymmetry-like first-order equations. 
I then turn to the topic of engineering vacua in the non-supersymmetric string models by constructing solutions that are supported by electric and magnetic fluxes and by providing evidence for their instability. 
Finally, I investigate brane-like solutions in the presence of tadpole potentials that yield both flux vacua with the isometries of supersymmetric branes and gravitational profiles that capture the backreaction of localized sources.

==> frontmatter/dedication.tex <==
%!TEX root = ../dissertation.tex
% dedication text

\begin{flushright}
To my parents, Rossana and Lorenzo,\\ my sister, Anna,\\ and my partner, Agata.
\end{flushright}


==> frontmatter/sns_page.tex <==
\thispagestyle{empty}
\newgeometry{top=0.2in, bottom=0.4in, includehead, includefoot}
\begin{center}
\includegraphics[width=2.43in]{figures/logo_SNS.pdf}  

\vspace{2.5cm}

{\Large Classe di Scienze\par}
\vspace{0.3cm}
{\Large Corso di perfezionamento in \par}
{\Large Fisica \par}
\vspace{0.3cm}
{\Large XXXVI ciclo \par}

\vspace{1.8cm}

{\Huge Spacetime aspects of \\ non-supersymmetric strings}	
	
\vspace{0.5cm}

%{Settore Scientifico Disciplinare \textbf{FIS/02}}
{\small SSD IS/02}

\vspace{2.5cm}
	
\begin{minipage}[t]{0.4\textwidth}
    \Large
    Candidate\par
    Salvatore Raucci\par
\end{minipage}
\hspace{0.1\textwidth}
\begin{minipage}[t]{0.4\textwidth}	
\hspace{1cm}
\end{minipage}

\vspace{1cm}

\begin{minipage}[t]{0.4\textwidth}
    \Large
    Advisor\par
    Augusto Sagnotti\par
\end{minipage}
\hspace{0.1\textwidth}
\begin{minipage}[t]{0.4\textwidth}				
    \Large
    Supervisor\par
    Guilherme L.~Pimentel\par
\end{minipage}

\vspace{1cm}

\vfill
{\large Academic year 2023--2024\par}
\end{center}

\restoregeometry

==> frontmatter/thanks.tex <==
%!TEX root = ../dissertation.tex
% the acknowledgments section

Writing the Acknowledgments section of a thesis is nearly as difficult as writing the thesis itself: how could I properly acknowledge all the people who had an influence on me during my PhD? This is clearly a losing challenge at the outset, so I have no other choice but to make the same mistake that everyone else makes: writing a list that is, unfortunately but necessarily, partial. I am certainly forgetting some people who have been instrumental in this path and have shaped my identity over the past few years.

First and foremost, I want to thank my parents, my grandparents, and my sister for giving me unlimited support over the years, without which this journey would have been impossible.
I have received love and support throughout these years from several people, among which I especially want to thank Antonio, Margherita, Francesco, Dario, Silvia, Cesare and Donatella for showing me how I want to age as a physicist, Darya and Gui for being an example of life and for their essential tips, and Beatriz for making me understand the joy of life.

Finally, I know of no words to adequately thank you, Agata. This journey has been a shared effort, and you are the true key in everything I do.

Moving to the academic subsection of the Acknowledgments, I want to start by thanking my supervisor, Augusto Sagnotti, for his guidance in this field and for being an example of academic integrity, perhaps the most important lesson one can learn from a PhD.
I have been lucky in having several \emph{informal supervisors} during these years: I am deeply grateful to Alessandro Tomasiello for always being available to discuss and for inspiring some of my work, Mariana Gra\~na for allowing me to live the most important months of this academic journey and for encouraging me in crucial moments, and Guilherme Pimentel for constant guidance during the last years of my PhD.

I also want to express my gratitude to Carlo Angelantonj, Chris Blair, Emilian Dudas, Miguel Montero, Jihad Mourad, Susha Parameswaran, Enrico Trincherini, and Irene Valenzuela for their support, which kept me going and helped me grow academically.
I am especially grateful to my two \emph{virtual postdocs}, Ivano Basile and Alvaro Herr\'{a}ez, for their constant help, especially during the tough periods, and for their impact on me as a researcher.

These Acknowledgments would be critically incomplete without thanking Craig Clark, Veronica Collazuol, Gabriele Di Ubaldo, Bernardo Fraiman, Nicolas Kovensky, Hector Parra de Freitas, Tom Westerdijk, and Chen Yang for the countless conversations about physics and non-physics that have at times shaped most of my days.
Finally, I want to mention several key people over the past four years: Roberta Angius, Fien Apers, Fabio Apruzzi, Rahel Baumgartner, Iosif Bena, Valentina Bevilacqua, Ralph Blumenhagen, Giuseppe Bogna, Bruno Bucciotti, Davide Bufalini, Jos\'e Calder\'on Infante, Federico Carta, Gabriele Casagrande, Davide Cassani, Alberto Castellano, Angela Corvino, Marco Costa, Niccol\`o Cribiori, Matilda Delgado, Giuseppe Dibitetto, Alon Faraggi, Anamaria Font, Fridrik Gautason, Dongsheng Ge, Silvia Georgescu, Joaquim Gomes, Alessandra Grieco, Shaun Hampton, Carlo Heissenberg, Oscar Henriksson, Nico Kleijne, Christian Kneissl, Adrien Kuntz, Johannes Lahnsteiner, Vittorio Larotonda, Giorgio Leone, Andrea Luzio, Andriana Makridou, Victoria Martin, Alessandro Mininno, Carmine Montella, Matteo Morittu, Niels Obers, Simon Pekar, Pietro Pelliconi, Eric Perlmutter, Nicolò Petri, Rahul Poddar, David Prieto, Mario Ramos Hamud, Filippo Revello, Nicole Righi, Nicol\`o Risso, Tom Rudelius, Marco Scalisi, Francesco Serra, Marco Serra, Charlotte Sleight, Watse Sybesma, Massimo Taronna, Gimmy Tomaselli, Dimitrios Toulikas, Vincent Van Hemelryck, Sonali Verma, Gonzalo Villa, Raphaela Wutte, Matteo Zatti, Fabio Zoratti, and all the other people that I am sure I am leaving out here. I deeply thank you, and if you are reading up to here and do not find yourself in the above list of names, please accept my sincere apologies. I deeply thank you, too.
